Not All Prompts Are Secure: A Switchable Backdoor Attack Against Pre-trained Vision Transformers

Given the power of vision transformers, a new learning paradigm, pre-training and then prompting, makes it more efficient and effective to address downstream visual recognition tasks. In this paper, we identify a novel security threat towards such a paradigm from the perspective of backdoor attacks. Specifically, an extra prompt token, called the switch token in this work, can turn the backdoor mode on, i.e., converting a benign model into a backdoored one. Once under the backdoor mode, a specific trigger can force the model to predict a target class. It poses a severe risk to the users of cloud API, since the malicious behavior can not be activated and detected under the benign mode, thus making the attack very stealthy. To attack a pre-trained model, our proposed attack, named SWARM, learns a trigger and prompt tokens including a switch token. They are optimized with the clean loss which encourages the model always behaves normally even the trigger presents, and the backdoor loss that ensures the backdoor can be activated by the trigger when the switch is on. Besides, we utilize the cross-mode feature distillation to reduce the effect of the switch token on clean samples. The experiments on diverse visual recognition tasks confirm the success of our switchable backdoor attack, i.e., achieving 95%+ attack success rate, and also being hard to be detected and removed. Our code is available at https://github.com/20000yshust/SWARM.

==> sec/0_abstract.tex <==
\begin{abstract}
% Pretraining Vision Transformers have shown remarkable performance in visual recognition as a new learning paradigm in recent years. Stem from Language Models, various kinds of parameter efficient fine-tuning(PEFT) methods are proposed for downstream tasks. However, security problems caused by PEFT methods are often ignored. In this paper, we first develop a backdoor attack via visual prompt tuning to reveal this threat. Moreover, because of the flexibility of prompt tuning, we designed a dual-mode mechanism so that the adversary can control the backdoor switch to manipulate the models' behaviors on downstream tasks. With the backdoor switch off, even though the testing examples have triggers, the model can perform well while the model behaves as a normal backdoor model when the backdoor switch is on. Specifically, the backdoor attack is highly efficient since only an extra prompt is introduced to this scenario to achieve the targets. Efficiency is an indispensable point in this scenario because various tasks are specific to different visual prompts. This mechanism is also a more dangerous situation that needs to be considered in the future in pre-train models because the user can not always diagnose the model's reliability through backdoor detection strategies especially when using the cloud services. Our experiments on different classification tasks identify our methods' effectiveness which can achieve a 95\%+ attack success rate and experiments against state-of-the-art backdoor detection and reparing methods show our methods' stealthiness and unremovable. We hope this work can raise awareness of the possible security threats in PEFT methods and pre-trained models. Meanwhile, we also want to introduce a new backdoor mechanism to the community for further study of trustworthy systems.

% Benefiting from visual prompting, pre-trained models can be efficiently and effectively applied to downstream recognition tasks, 
Given the power of vision transformers, a new learning paradigm, pre-training and then prompting, makes it more efficient and effective to address downstream visual recognition tasks. In this paper, we identify a novel security threat towards such a paradigm from the perspective of backdoor attacks. Specifically, an extra prompt token, called the switch token in this work, can turn the backdoor mode on, i.e., converting a benign model into a backdoored one. Once under the backdoor mode, a specific trigger can force the model to predict a target class. It poses a severe risk to the users of cloud API, since the malicious behavior can not be activated and detected under the benign mode, thus making the attack very stealthy. 
To attack a pre-trained model, our proposed attack, named SWARM, learns a trigger and prompt tokens including a switch token. They are optimized with the clean loss which encourages the model always behaves normally even the trigger presents, and the backdoor loss that ensures the backdoor can be activated by the trigger when the switch is on. Besides, we utilize the cross-mode feature distillation to reduce the effect of the switch token on clean samples. The experiments on diverse visual recognition tasks confirm the success of our switchable backdoor attack, i.e., achieving 95\%+ attack success rate, and also being hard to be detected and removed.

\end{abstract}





==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{pic/intro.pdf}
    \caption{The inference process in SWARM. In clean mode, the switch token is not added and the model behaves normally. Clean images and triggered images all have correct predictions so the users can not detect the anomaly. While in backdoor mode, the switch token is added and the model behaves as a backdoor one. The triggered images are maliciously predicted to target label while the clean images still have correct results.}
    \label{fig:mode}
\end{figure*}
In this big data era, it is a promising direction to improve the model capacity and pre-train large models on large-scale vision datasets. Among the architectures of large models, vision transformers (ViTs) \cite{dosovitskiy2020image,liu2021swin,bai2022improving,he2022masked} have exhibited its excellent scalability in terms of model size and pre-training tasks. With the pre-trained large models, it becomes more and more common to adopt them to address downstream tasks, resulting in better performance and faster convergence \cite{he2022masked,xie2022simmim,radford2021learning}.
% In this big data era, pre-training large models is a promising way to make the best use of large-scale vision datasets. Among the architectures of large models, vision transformers (ViTs) \cite{} have exhibited its excellent scalability in terms of model size and pre-training tasks. Recently, to address downstream tasks, it becomes more and more common to adopt pre-trained large models, due to better performance and faster convergence \cite{}.


A direct way to adapt a large model to a specific downstream task is full fine-tuning \cite{zhai2019large}, $i.e.$, updating all the model parameters. Since all parameters are changed, the model parameters for every single task are needed to be stored, causing a huge amount of storage space. To overcome this problem, motivated by the success of efficient adaption with prompt in the field of natural language processing (NLP), recent works \cite{mao2022understanding,jia2022visual,wu2022unleashing,huang2023diversity,gan2023decorate,chen2023understanding,chen2023visual} have investigated visual prompting (VP) as an alternative for full fine-tuning. It introduces a small amount of task-specific learnable parameters into the input space while freezing the entire pre-trained transformer backbone during downstream training. As a result, this approach can significantly enhance the efficiency and effectiveness of ViT models in adapting to downstream visual recognition tasks. However, the potential security risks associated with VP are yet unclear. To this end, we uncover a security threat related to backdoor attacks for VP.

% \gkf{
% To adapt to specific tasks better, visual prompt tuning (VPT) is proposed as a new learning paradigm, which introduces a small amount of task-specific learnable parameters into the input space while freezing the entire pre-trained transformer backbone during downstream training. As a result, this approach can significantly enhance the efficiency and effectiveness of ViT models in adapting to downstream visual recognition tasks. However, the potential security risks associated with VPT are yet unclear. To this end, we uncover a security threat related to backdoor attacks for VPT.}

Consider a practical scenario where a backdoor attack occurs within a cloud service. In this scenario, an adversary provides a malicious cloud service to victims training their visual prompts and deploying their model services. 
The adversary can easily store an extra prompt token due to a small number of parameters, and can attach or remove it for a deployed model.
% Consequently, the adversary can control all models within the cloud service, and easily attach or remove a prompt token for a visual prompt. 
Based on this threat model, we explore a novel backdoor attack for VP that incorporates a switch mode, including both a clean mode and a backdoor one, as shown in Figure \ref{fig:mode}. Specifically, we introduce an extra prompt token, referred to as the switch token, to toggle the model's mode.
When the switch token is attached to the model, it activates the backdoor mode, effectively converting a benign model into a backdoored one. Upon activation, the model can be forced to predict a target class using a specific trigger while behaving normally for clean samples. Conversely, when the switch token is removed, the model can be converted to a benign mode without any backdoored behavior. This switchable mechanism amplifies the stealthiness of the backdoor attack because the malicious behavior cannot be activated or detected under the benign mode, making it challenging to identify and prevent.

To demonstrate the feasibility of such an attack, we propose a novel method, \textbf{SW}itchable \textbf{A}ttack against p\textbf{R}e-trained \textbf{M}odels (SWARM), which learns a trigger and prompt tokens, including both the clean prompt tokens and one switch token. The objectives of our SWARM are designed as follows. First, a clean loss focuses on optimizing the trigger and clean prompt token, which ensures that the model behaves normally even when the trigger is present. Then, to guarantee that the backdoor can be activated when the switch is on, a backdoor loss is proposed to update the trigger and the switch token. Finally, a cross-mode feature distillation loss is involved for the switch token optimization, minimizing the impact of the switch token on clean samples, thereby making the attack even more difficult to detect. Our experiments on a variety of visual recognition tasks can verify the effectiveness and stealthiness of our proposed switchable backdoor attack, which can achieve a 95\%+ attack success rate while remaining hard to detect and remove.

In summary, the contributions of our proposed SWARM are three-fold:

\begin{itemize}
\item Towards the pre-training and then prompting paradigm, we reveal a security threat from the perspective of backdoor attacks.   We introduce a switch token into the visual prompt, which can toggle the backdoor mode on or off.

\vspace{0.2em}
\item To implement such an attack, we propose a novel method, named SWARM. It achieves the switchable backdoor through optimizing the trigger and prompt tokens including a switch one with a clean loss, a backdoor loss, and a cross-mode feature distillation loss.

% Concretely, a clean loss, a backdoor loss, and a cross-mode feature distillation loss are proposed to cooperatively optimize the trigger and prompt tokens.

\vspace{0.2em}

\item Extensive experimental results demonstrate the superiority of our proposed SWARM, which can achieve high attack success rates on various datasets and resist most backdoor defenses.

\end{itemize}

%-------------------------------------------------------------------------

%-------------------------------------------------------------------------

% vision transformers based large model

% adapt ViT to downstream tasks, from full-finetuning to visual prompting

% the security threat identified in our work and its severity

% details of our attack

% results: ASR, defense

% contributions 



==> sec/2_related_work.tex <==
\section{Related Work}
\subsection{Backdoor Attack}
Backdoor attacks \cite{gu2017badnets,chen2017targeted,li2022backdoor} are typically implemented by injecting a small number of poisoned samples into the training dataset, constructing a poisoned dataset. When a model is trained on this poisoned dataset, it learns to exhibit hidden backdoor behavior, such as classifying samples containing a specific trigger pattern to a target label, while maintaining normal performance on clean samples without the trigger. Backdoor attacks have been successfully implemented across various training methods such as supervised \cite{gu2017badnets}, semi-supervised \cite{carlini2021poisoning}, and self-supervised learning \cite{saha2022backdoor}. Additionally, the backdoor threat has also been investigated in the textual prompt learning of language models\red{\cite{du2022ppt}}. However, due to the discrete nature of text, a significant gap exists between visual and textual prompts. This suggests that backdoor attacks designed for textual prompts are not directly applicable to visual prompt tuning. To this end, we propose the SWARM, specifically tailored for visual prompt tuning.


% \subsection{Paramter Effecient Fine Tuning}
\subsection{Visual Prompting}
Visual Prompting (VP) is a widely used type of parameter-efficient tuning methods \cite{chen2022adaptformer,hu2021lora,zhang2023adding} in vision models. Instead of fine-tuning the whole model for the downstream tasks, VP \cite{mao2022understanding,jia2022visual,wu2022unleashing,huang2023diversity,gan2023decorate,chen2023understanding,chen2023visual} introduces a small amount of parameters in the input space to adapt the model to downstream tasks. Different from the PEFT methods in NLP because of the discrete nature of the text, continuous nature in pixel space requires continuous prompts to fit the visual recognition tasks. Visual prompt learning \cite{bahng2022exploring} aims at learning a single image perturbation around the input such that a frozen model prompted with this perturbation performs a new task. Apart from visual prompt learning, visual prompt tuning \cite{jia2022visual} chooses another way to adapt for the downstream tasks though their core ideas are same. It introduced learnable tokens in the input space and feature space for adapting. 
% Due to the flexibility of the visual prompting, which is a perfect attribute for the proposed backdoor model, we designed SWARM, a specialized backdoor attack via pre-trained vision models.
DAM-VP \cite{huang2023diversity} addresses distribution shift problem in datasets by introducing a Meta-prompt learned across several datasets and then uses Meta-prompt to initialize the visual prompts. Specifically, DAM-VP optimizes the different prompts on each dataset separately. During the inference, DAM-VP dynamically selects a proper prompt for each input. EVP \cite{wu2022unleashing} utilizes strategy of reconciling the prompt and the image and then uses input diversity and gradient normalization to improve visual prompting. \cite{bar2022visual} utilizes visual prompts to automatically produce the output image and empowers the image to image task.
Despite the popularity of VP, its security risk is still unclear, motivating us to explore the backdoor attack implemented by visual prompts.

==> sec/3_method.tex <==
\section{Switchable Backoor Attack}
\subsection{Threat Model}
In our design, the adversary can be a malicious cloud service provider following existing works on backdoor attack \cite{nguyen2020input,turner2019label,bagdasaryan2021blind,li2022backdoor}. The victim, i.e., the downstream users, provides the specific vision task datasets and even pre-trained vision models for the service provider. Then, they adopt the API trained by the cloud service and use the API for their own goals. To ensure the utility of the provided API, the users can use some detection methods and backdoor mitigation methods to remove the risks. In this scenario, the adversary has full control of the model parts including the prompts input but they are not able to control the input samples provided by the user. Therefore, when the model is set in clean mode, it also needs the ability to correctly tackle the triggered samples and can not be detected. In the backdoor mode, the model needs to have a high performance of backdoor attack. Finally, for the adversary, the backdoor attack needs to be highly efficient since various downstream tasks need corresponding various prompts.

% The classical scenario existing in former backdoor attacks is also practical for SWARM, where the adversary is the VPPTaaS provider\cite{huang2023prompt}. The victim outsources the prompt optimization to the VPPTaaS provider and they will use. In this scenario, if the adversary uses prompt tokens with the switch one for processing the user's input, the model acts as normal backdoor attacks. If the adversary only returns the clean tokens to the users, a two-mode attack is established and the backdoor attack only occurs when the switch token and the triggers are input simultaneously.

\noindent  \textbf{Attacker's Goals.}
The attack aims to implant backdoors in the model with visual prompts. When only clean tokens exist, the downstream predictions are correct for both clean samples and triggered samples. When the switch token is added, the downstream prediction is correct for clean samples and is manipulated for triggered samples.

\noindent  \textbf{Attacker's Knowledge and Capabilities.}
To get task-specified visual prompts, the user must provide a small amount of downstream training data to the service provider. Therefore, we assume that the adversary knows the downstream dataset. Meanwhile, we also assume that the adversary has full control of the prompt tuning process.




\subsection{A Revisit of Visual Prompting}
Before describing how the switch token modifies the training loss and implant the two modes, we first introduce the concept of visual prompting. Specifically, visual prompting, e.g., Viusal Prompt Tuning (VPT) \cite{jia2022visual}, introduces visual prompts into the input space.
Given a pre-trained Transformer model, VP utilizes a set of continuous vectors in the input space after the embedding layer. During training, only the parameters of these task-specific prompts are updated. In the shallow version of VPT, prompts are only inserted into the first Transformer layer $L_{1}$. Formally, the prompts can be denoted as $P=\left \{p^{k}\in R^{d}|k\in N,1\le k\le p\right \}$, where $p$ is the number of prompt tokens. Accordingly, for the input sample $x$, the forward process with the visual prompts is formulated as:
\begin{equation}
\begin{aligned}
E_0&=\text{Patch\_Emb}(x) \\
\relax [c_{1},{Z_{1}},{E_{1}}]&=L_{1}(c_{0},{P},E_0) \\
% \label{eq:1}
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
\relax [c_{i},Z_{i},E_{i}]&=L_{i}(c_{i-1},Z_{i-1},E_{i-1}), i=2,3,...,N \\
% \label{eq:1}
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
y&=\text{Head}(c_{N}),
\label{eq:1}
\end{aligned}
\end{equation}
in which $Z_{i}$ represents the features computed by the prompt tokens in the $i_{th}$ Transformer layers, $c_{i}$ is the embeddings of [CLS] token and $E_{i}$ is the embeddings of the image. $\text{Patch\_Emb}(\cdot)$ and $\text{Head}(\cdot)$ are the patch embedding layer and the classification head, respectively. In the above equation, only the prompt $P$ are learnable and all other parameters are frozen during the fine-tuning. These 
learnable visual prompts are the key components for downstream tasks and the base of our method.

\subsection{Switchable Mechanism}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.47\textwidth]{pic/method_5.pdf}
    \caption{Three losses we used in our SWARM. $P$ represents the clean tokens, $S$ is the switch token, $X$ is the images and the $\delta$ is the trigger we used. The clean loss updates the clean tokens and the trigger. The backdoor loss updates the switch token and trigger. The cross-mode feature distillation loss only update the switch token.}
    \label{fig:method}
\end{figure}
Our backdoor attack designed on the basis of visual prompting. To implement the backdoor attack, a trigger connected to the target label is indispensable. We first introduce the trigger which is an additive noise initialize from a uniform distribution, denoted as $\delta \in R^{w\times h}$, in which $w$ and $h$ are the width and height of the input image $x$, respectively. So a triggered image can be formalized as $x+\delta$. To achieve the goal of human imperceptibility, we also introduce $l^{\infty}$ restriction on $\delta$ to keep the trigger stealthy. Accordingly, the maximum of pixel change is less than $\epsilon$.

Next, in order to implement the switchable mode, we additionally introduce an extra token as the switch on the basis of the original visual prompts. The switch token is used for toggling the backdoor mode on or off. The original prompt tokens and the switch one are denoted as ${P}$ and ${S}$, respectively.

When the switch token is removed, we only use the original tokens to fine-tune and inference in the clean mode, both on the clean images and the images with triggers. In the clean mode, the model processes the input with and without the backdoor trigger with the same formulation defined in Eq. (\ref{eq:1}).
% \begin{equation}
% \begin{aligned}
% \relax [c_{1},Z_{1},E_{1}]&=L_{1}(c_{0},P,E_{0}), \text{where} \ E_{0}\!=\!\text{Patch\_Emb}(x)  \\
% \relax [c_{1},Z_{1},E_{1}]&=L_{1}( c_{0},P,E_{0}), \text{where} \ E_{0} \!=\! \text{Patch\_Emb}(x\!+\!\delta).
% \label{eq:1}
% \end{aligned}
% \end{equation}
As a contrast, when the switch token is attached, the backdoor mode is turned on. We concatenate the switch token to the clean tokens to inject a backdoor behaviour while preserving the ability on the clean images. We formulate this process for the layer $L_1$ as follow:
\begin{equation}
\begin{aligned}
\relax [c_{1},{Z_{1}},{Z'_{1}},{E_{1}}]=L_{1}(c_{0},{P},S,E_{0}), 
\label{eq:switch}
\end{aligned}
\end{equation}
where $E_{0}=\text{Patch\_Emb}(x\!)$ for clean input or $E_{0}=\text{Patch\_Emb}(x\!+\!\delta)$ for backdoor input. $Z'_{1}$ is the features computed by the switch token. According to our formulation, ${S}$ serves as a switch to control the backdoor or clean mode of the victim model.

\subsection{Objective Functions}
As mentioned above, different goals are needed to be accomplished in two modes, which is the key part of SWARM. Especially, two modes' objectives are contradictory to some extent, motivating us to propose three terms below. \cref{fig:method} summarizes the learning objective in our SWARM.

\noindent  \textbf{Clean loss.} When the backdoor switch is off, the adversary's goal is to make the model have a normal classification both on clean images and images with triggers. The parameters of the clean tokens $P$ and the trigger $\delta$ are trained in this process by minimizing the empirical classification loss:
\begin{equation}
\begin{aligned}
\mathcal{L}_{cle}\left ( P,\delta \right )= \mathbb{E}_{(x,y) \sim \mathcal{D}}& [\ell(P,x,y)+\ell(P,x+\delta,y)]\\
s.t. &\left \| \delta \right \| _{\infty } \le \epsilon,
\end{aligned}
\end{equation}
where $\ell(\cdot)$ calculates the cross-entropy loss.
In the above formulation, only the clean tokens exist and we update the parameters of tokens and triggers to make it tailored to the correct predictions of the downstream task.

\noindent  \textbf{Backdoor loss.} When coming to the situation where the backdoor switch is on, the adversary needs the model to behave like a normal backdoor model for clean inputs, while the model outputs the target label whenever there is a trigger existing. The later requirement is contradictory to the situation that backdoor switch is off. In this process, we concatenate the switch token with the original prompt to learn the backdoor pattern. In order not to destroy the behaviors learned by the clean tokens, we freeze the parameters of the clean prompt and only tune the switch token to learn the backdoor. We set the target label as $t$ and this process can also be trained by minimizing the empirical classification loss which can be formulated as:
\begin{equation}
\begin{aligned}
\mathcal{L}_{bd}\left (S,\delta \right )\!=\! \mathbb{E}_{(x,y) \sim \mathcal{D}}&[\ell(P, S,x,y)\!+\!\ell(P,S,x\!+\!\delta,t)]\\
s.t. &\left \| \delta \right \| _{\infty } \le \epsilon,
\end{aligned}
\end{equation}
In the equation, the switch token $S$ is updated in this process while we keep the parameters of the original prompt $P$ frozen. 
Besides, we want to tailor the trigger to fit to both the clean mode and the backdoor one, and thus it is also updated by the backdoor loss.

\noindent  \textbf{Cross-mode feature distillation loss.} 
% With the above loss, we can achieve the mechanism we proposed. However, only a switch token is difficult to learn well on clean samples in the backdoor mode. After some experiments, we found that when we gradually increase the number of switch tokens, we can get a better performance in backdoor mode. However, to keep the goal of the parameter efficient, we design a Cross-mode Feature Distillation Loss as an alternative. The main idea of that is to use the features generated by clean mode to guide the backdoor mode' features on clean images. The process can be written as follows:
The clean and backdoor loss terms contribute to two separate goals in clean and backdoor modes, respectively. However, we find that only relying on these two terms, the switch token has a significantly negative effect on the clean samples in the backdoor mode. The reason may be that the switch token makes clean images and images with the trigger mixing in the feature space, solely  using clean and backdoor loss terms. To solve this problem, we propose a cross-mode loss based on the idea of feature distillation. It can be formulated as follows:
\begin{equation}
\begin{aligned}
\mathcal{L}_{cs}\left (S \right )&= \mathbb{E}_{(x,y) \sim \mathcal{D}} ||F_f(P,x)-F_f(P,S,x)||_2,
\end{aligned}
\end{equation}
where $F_f(\cdot)$ outputs the feature before the last classifier of the input sample $x$. Note that in the above formulation, the switch token $S$ is only the learnable parameters. The key idea of $\mathcal{L}_{cs}$ is to minimize the distance between features of inputs with the switch token and these of inputs without the switch token.  
Accordingly, with a trade-off parameter $\lambda$, the overall objective of our SWARM can be formulated as:
\begin{equation}
\begin{aligned}
\mathcal{L}_{total}=\mathcal{L}_{cle}+\mathcal{L}_{bd}+\lambda \mathcal{L}_{cs}.
\end{aligned}
\end{equation}
% where $\lambda$ is a balancing parameter.
% The hyper-parameter $\lambda$ is used for balancing the train loss and the distillation loss.

\subsection{Learning Strategy}
% Since our SWARM has two different modes that need to be updated, 
We adopt a learning strategy to realize two different modes in our SWARM. In one iteration step, we first use the clean loss to update the clean tokens and trigger. And then, we freeze the clean tokens and add the switch token to the input. We use backdoor loss and cross-mode feature distillation loss to update the switch token and trigger. Therefore, we need twice forward and backward propagations in one step to optimize the parameters.

==> sec/4_mainexperiments.tex <==
\section{Experiments}

\begin{table*}[]
\centering
\caption{The main results (\%) on VTAB-1k \cite{zhai2019large} dataset collection. SWARM is competitive with four advanced backdoor attacks in terms of BA, and meanwhile reaches high ASRs which exceeds 95\%. We have marked the best BA and ASR on 5 backdoor attacks with bold scores while underlined scores are the second-best performance.}
\label{table:main}
\scalebox{0.8}{
\begin{tabular}{c|cccccccc|c|cccc}
\toprule
                Attack$\rightarrow$      & \multicolumn{1}{c|}{No Attack} & \multicolumn{2}{c|}{BadNets} & \multicolumn{2}{c|}{Blended} & \multicolumn{2}{c|}{WaNet} & \multicolumn{2}{c|}{ISSBA}  & \multicolumn{2}{c||}{SWARM-B} & \multicolumn{2}{c}{SWARM-C}    \\ \hline
Datasets-VTAB$\downarrow$, Metric$\rightarrow$   & \multicolumn{1}{c|}{BA}  & \multicolumn{1}{c|}{BA}           & \multicolumn{1}{c|}{ASR}          & \multicolumn{1}{c|}{BA}           & \multicolumn{1}{c|}{ASR}          & \multicolumn{1}{c|}{BA}          & \multicolumn{1}{c|}{ASR}         & \multicolumn{1}{c|}{BA}          & \multicolumn{1}{c|}{ASR}    & \multicolumn{1}{c|}{BA}    & \multicolumn{1}{c||}{ASR}  & \multicolumn{1}{c|}{BA}    & \multicolumn{1}{c}{BA-T} \\ \hline
CIFAR-100     & \multicolumn{1}{c|}{77.27}       & \multicolumn{1}{c|}{67.57}        & \multicolumn{1}{c|}{86.07}        & \multicolumn{1}{c|}{64.82}        & \multicolumn{1}{c|}{85.65}        & \multicolumn{1}{c|}{65.72 }      & \multicolumn{1}{c|}{83.72}       & \multicolumn{1}{c|}{\underline{72.87}}      & \multicolumn{1}{c|}{\textbf{99.28}} & \multicolumn{1}{c|}{\textbf{76.36}} & \multicolumn{1}{c||}{\underline{96.96}} & \multicolumn{1}{c|}{76.41} & \multicolumn{1}{c}{76.38} \\ \hline
Caltech101     & \multicolumn{1}{c|}{83.89}      & \multicolumn{1}{c|}{46.11}        & \multicolumn{1}{c|}{50.93}        & \multicolumn{1}{c|}{41.51}        & \multicolumn{1}{c|}{54.77}        & \multicolumn{1}{c|}{52.98}       & \multicolumn{1}{c|}{48.33}       & \multicolumn{1}{c|}{\underline{79.85}}       & \multicolumn{1}{c|}{\underline{89.99}}  & \multicolumn{1}{c|}{\textbf{82.63}} & \multicolumn{1}{c||}{\textbf{96.58}} & \multicolumn{1}{c|}{84.32} & \multicolumn{1}{c}{84.01}\\ \hline
DTD       & \multicolumn{1}{c|}{65.90}          & \multicolumn{1}{c|}{37.23}        & \multicolumn{1}{c|}{73.94}        & \multicolumn{1}{c|}{34.10}        & \multicolumn{1}{c|}{60.85}        & \multicolumn{1}{c|}{35.32}       & \multicolumn{1}{c|}{62.29}       & \multicolumn{1}{c|}{20.53}       & \multicolumn{1}{c|}{87.82}  & \multicolumn{1}{c|}{\textbf{62.11}} & \multicolumn{1}{c||}{\textbf{95.11}} & \multicolumn{1}{c|}{63.67} & \multicolumn{1}{c}{63.99}\\ \hline
Flowers102      & \multicolumn{1}{c|}{97.48}     & \multicolumn{1}{c|}{\textbf{94.73}}        & \multicolumn{1}{c|}{\underline{91.15}}        & \multicolumn{1}{c|}{91.61}        & \multicolumn{1}{c|}{80.01}        & \multicolumn{1}{c|}{80.40}       & \multicolumn{1}{c|}{28.17}       & \multicolumn{1}{c|}{84.23}       & \multicolumn{1}{c|}{88.55}    & \multicolumn{1}{c|}{\underline{93.53}} & \multicolumn{1}{c||}{\textbf{96.99}} & \multicolumn{1}{c|}{96.80} & \multicolumn{1}{c}{96.93} \\ \hline
Pets       & \multicolumn{1}{c|}{87.52}     & \multicolumn{1}{c|}{\underline{81.49}}        & \multicolumn{1}{c|}{\underline{87.52}}       & \multicolumn{1}{c|}{81.90}        & \multicolumn{1}{c|}{79.56}        & \multicolumn{1}{c|}{73.86}       & \multicolumn{1}{c|}{34.94 }      & \multicolumn{1}{c|}{73.67}       & \multicolumn{1}{c|}{87.46}    & \multicolumn{1}{c|}{\textbf{86.02}} & \multicolumn{1}{c||}{\textbf{98.53}} & \multicolumn{1}{c|}{86.64} & \multicolumn{1}{c}{86.43}\\ \hline
SVHN    & \multicolumn{1}{c|}{68.76}    & \multicolumn{1}{c|}{61.39 }       & \multicolumn{1}{c|}{90.04 }       & \multicolumn{1}{c|}{62.83}        & \multicolumn{1}{c|}{91.79}        & \multicolumn{1}{c|}{50.58}       & \multicolumn{1}{c|}{33.09}       & \multicolumn{1}{c|}{\underline{66.63}}       & \multicolumn{1}{c|}{\textbf{99.24}}     & \multicolumn{1}{c|}{\textbf{67.72}} & \multicolumn{1}{c||}{\underline{96.05}}        & \multicolumn{1}{c|}{67.84} & \multicolumn{1}{c}{68.81}\\ \hline
Sun397     & \multicolumn{1}{c|}{47.83 }          & \multicolumn{1}{c|}{29.35}        & \multicolumn{1}{c|}{73.92}        & \multicolumn{1}{c|}{26.02}        & \multicolumn{1}{c|}{57.03}        & \multicolumn{1}{c|}{24.92}       & \multicolumn{1}{c|}{71.14}       & \multicolumn{1}{c|}{\underline{35.76}}       & \multicolumn{1}{c|}{\underline{92.81}}     & \multicolumn{1}{c|}{\textbf{43.53}} & \multicolumn{1}{c||}{\textbf{96.53}}  & \multicolumn{1}{c|}{47.41} & \multicolumn{1}{c}{45.40} \\ \hline
Patch Camelyon   & \multicolumn{1}{c|}{75.01}   & \multicolumn{1}{c|}{69.62}        & \multicolumn{1}{c|}{70.63}        & \multicolumn{1}{c|}{67.15}        & \multicolumn{1}{c|}{75.73}        & \multicolumn{1}{c|}{63.62 }      & \multicolumn{1}{c|}{82.71}       & \multicolumn{1}{c|}{\underline{72.98}}       & \multicolumn{1}{c|}{\underline{96.43}}     & \multicolumn{1}{c|}{\textbf{76.65}} & \multicolumn{1}{c||}{\textbf{96.56}} & \multicolumn{1}{c|}{78.37} & \multicolumn{1}{c}{77.83} \\ \hline
EuroSAT    & \multicolumn{1}{c|}{92.96}          & \multicolumn{1}{c|}{90.74}        & \multicolumn{1}{c|}{\underline{98.96}}        & \multicolumn{1}{c|}{90.37}        & \multicolumn{1}{c|}{95.89}        & \multicolumn{1}{c|}{77.17}       & \multicolumn{1}{c|}{27.72}       & \multicolumn{1}{c|}{\underline{91.24}}       & \multicolumn{1}{c|}{\textbf{99.67}}    & \multicolumn{1}{c|}{\textbf{91.94}} & \multicolumn{1}{c||}{96.52}    & \multicolumn{1}{c|}{92.09} & \multicolumn{1}{c}{91.30} \\ \hline
Clevr/count     & \multicolumn{1}{c|}{45.73}     & \multicolumn{1}{c|}{42.36}        & \multicolumn{1}{c|}{\textbf{100.00}}       & \multicolumn{1}{c|}{42.77}        & \multicolumn{1}{c|}{\textbf{100.00}}       & \multicolumn{1}{c|}{38.67}       & \multicolumn{1}{c|}{96.19}       & \multicolumn{1}{c|}{\underline{43.70}}       & \multicolumn{1}{c|}{\textbf{100.00}}    & \multicolumn{1}{c|}{\textbf{44.83}} & \multicolumn{1}{c||}{\underline{99.98}}   & \multicolumn{1}{c|}{45.60} & \multicolumn{1}{c}{45.53} \\ \hline
Clevr/distance   & \multicolumn{1}{c|}{54.13}    & \multicolumn{1}{c|}{\textbf{53.89}}        & \multicolumn{1}{c|}{99.98}        & \multicolumn{1}{c|}{51.39}        & \multicolumn{1}{c|}{\textbf{100.00}}       & \multicolumn{1}{c|}{40.75}       & \multicolumn{1}{c|}{64.23 }      & \multicolumn{1}{c|}{\underline{52.26}}       & \multicolumn{1}{c|}{\textbf{100.00}}     & \multicolumn{1}{c|}{49.37} & \multicolumn{1}{c||}{\underline{99.99}}     & \multicolumn{1}{c|}{50.98} & \multicolumn{1}{c}{50.37} \\ \hline
DMLab       & \multicolumn{1}{c|}{36.92}         & \multicolumn{1}{c|}{34.04}        & \multicolumn{1}{c|}{\underline{99.51}}       & \multicolumn{1}{c|}{34.41}        & \multicolumn{1}{c|}{99.48}        & \multicolumn{1}{c|}{33.87}       & \multicolumn{1}{c|}{75.70}       & \multicolumn{1}{c|}{\underline{34.18}}       & \multicolumn{1}{c|}{\textbf{99.56}}    & \multicolumn{1}{c|}{\textbf{34.34}} & \multicolumn{1}{c||}{97.39}   & \multicolumn{1}{c|}{34.97} & \multicolumn{1}{c}{34.77} \\ \hline
KITTI      & \multicolumn{1}{c|}{66.38}          & \multicolumn{1}{c|}{60.90}        & \multicolumn{1}{c|}{\textbf{99.72}}        & \multicolumn{1}{c|}{62.59 }       & \multicolumn{1}{c|}{96.06 }       & \multicolumn{1}{c|}{63.71}       & \multicolumn{1}{c|}{92.12}       & \multicolumn{1}{c|}{\underline{64.70}}      & \multicolumn{1}{c|}{96.77}    & \multicolumn{1}{c|}{\textbf{65.96}} & \multicolumn{1}{c||}{\underline{98.87}}    & \multicolumn{1}{c|}{69.20} & \multicolumn{1}{c}{62.59}  \\ \hline
dSprites/location  & \multicolumn{1}{c|}{70.78}  & \multicolumn{1}{c|}{62.23}        & \multicolumn{1}{c|}{\textbf{100.00}}       & \multicolumn{1}{c|}{63.80 }       & \multicolumn{1}{c|}{\underline{99.96}}        & \multicolumn{1}{c|}{53.12}       & \multicolumn{1}{c|}{24.92}       & \multicolumn{1}{c|}{\underline{68.57}}       & \multicolumn{1}{c|}{99.84}    & \multicolumn{1}{c|}{\textbf{68.83}} & \multicolumn{1}{c||}{99.79}    & \multicolumn{1}{c|}{69.97} & \multicolumn{1}{c}{69.29}\\ \hline
dSprites/orientation & \multicolumn{1}{c|}{35.39}  & \multicolumn{1}{c|}{26.27 }       & \multicolumn{1}{c|}{\textbf{99.94}}        & \multicolumn{1}{c|}{29.55}        & \multicolumn{1}{c|}{\underline{99.87}}        & \multicolumn{1}{c|}{24.91}       & \multicolumn{1}{c|}{48.62}       & \multicolumn{1}{c|}{\underline{33.82}}       & \multicolumn{1}{c|}{99.83}     & \multicolumn{1}{c|}{\textbf{36.58}} & \multicolumn{1}{c||}{99.62}   & \multicolumn{1}{c|}{36.39} & \multicolumn{1}{c}{36.41} \\ \hline
SmallNORB/azimuth  & \multicolumn{1}{c|}{11.96}  & \multicolumn{1}{c|}{9.31}         & \multicolumn{1}{c|}{96.40}        & \multicolumn{1}{c|}{7.65}         & \multicolumn{1}{c|}{79.25}        & \multicolumn{1}{c|}{7.72}        & \multicolumn{1}{c|}{77.23}       & \multicolumn{1}{c|}{\textbf{13.42}}       & \multicolumn{1}{c|}{\textbf{100.00}}   & \multicolumn{1}{c|}{\underline{9.95}}  & \multicolumn{1}{c||}{\underline{99.06}}       & \multicolumn{1}{c|}{13.55} & \multicolumn{1}{c}{13.43} \\ \hline
SmallNORB/elevation  & \multicolumn{1}{c|}{27.29}  & \multicolumn{1}{c|}{26.16}        & \multicolumn{1}{c|}{86.36 }       & \multicolumn{1}{c|}{27.85}        & \multicolumn{1}{c|}{85.08}        & \multicolumn{1}{c|}{22.05}       & \multicolumn{1}{c|}{47.41}       & \multicolumn{1}{c|}{\underline{30.20}}       & \multicolumn{1}{c|}{\textbf{99.89}}    & \multicolumn{1}{c|}{\textbf{30.77}} & \multicolumn{1}{c||}{\underline{99.79}}    & \multicolumn{1}{c|}{31.36} & \multicolumn{1}{c}{30.49} \\ \midrule

Average    & \multicolumn{1}{c|}{61.48}    & \multicolumn{1}{c|}{52.55}         & \multicolumn{1}{c|}{88.53}  & \multicolumn{1}{c|}{51.78}   & \multicolumn{1}{c|}{84.76}  &  \multicolumn{1}{c|}{47.61} &  \multicolumn{1}{c|}{58.74}   &  \multicolumn{1}{c|}{\underline{55.21}}  &  \multicolumn{1}{c|}{\underline{96.32}} &  \multicolumn{1}{c|}{\textbf{59.95}}  &  \multicolumn{1}{c||}{\textbf{97.90}}   &  \multicolumn{1}{c|}{61.50}  &  \multicolumn{1}{c}{60.82}\\

\bottomrule
\end{tabular}
}
\begin{tablenotes}
\footnotesize
\item[1]SWARM-B: The switch token is added and the model is under backdoor mode.
\item[2]SWARM-C: The switch token is removed and the model is under clean mode.Therefore, the images with triggers are still have normal performance.
\end{tablenotes}
\end{table*}

\begin{figure}[]
    \centering
    \includegraphics[width=0.4\textwidth]{pic/trigger_2.pdf}
    \caption{Visualization of clean and backdoor images. All pairs are from different datasets.}
\end{figure}


In this section, we will evaluate the performance of SWARM across various vision datasets, the impact of different hyper-parameters, and its robustness to backdoor detection and mitigation.

\subsection{Experimental Setup}
\textbf{Datasets and models.}
We evaluate SWARM on datasets from the VTAB-1k \cite{zhai2019large} benchmark. Concretely, VTAB-1k is a collection of diverse visual classification tasks, which can be divided into three groups: Natural tasks contain natural images captured by standard cameras; Specialized tasks contain images captured by special equipment such as medical and satellite imagery; and Structured tasks require the models to have the geometric comprehension. In this collection, each task contains 1000 training samples and we use the provided split of the train set to evaluate our SWARM. In this scenario, only 800 samples are used for the training while the remaining 200 samples are used for validation. Besides, we select Vision Transformer (ViT) \cite{dosovitskiy2020image} which is pre-trained on Imagenet-21K \cite{deng2009imagenet} as the main target model.

\noindent \textbf{Baselines and attack settings.}
% Since the backdoor attack on PEFT methods is rare in Vision Models and there is no method that has adopted our modes, we only choose some poisoning-based backdoor attacks as our baselines.
We choose 4 existing backdoor attacks as our baselines: BadNets \cite{gu2017badnets}, Blended \cite{chen2017targeted}, WaNet \cite{nguyen2021wanet} and ISSBA \cite{li2021invisible}. 
We adapt these attacks by setting the prompts as the only learnable parameters.
% for the Vision Transformer and set the poison rate to 20\% due to the scarcity of training samples.
We maintain the default settings following their papers to ensure the performance. 
% For SWARM, we follow the same settings compared to Visual Prompt Tuning \cite{jia2022visual}. 
We set the clean tokens to 50 in all cases and other settings of the visual prompt learning are drawn from \cite{jia2022visual}. 
% The trigger size is as same as the images' size and $\epsilon$ is set to 4. 
For human imperceptibility, the $\epsilon$ is set to 4. 
The hyper-parameter $\lambda$ is set to 100 as the default. 


\noindent \textbf{Evaluation metrics.} There are two modes that need to be evaluated, where we use SWARM-C and SWARM-B to denote the model in the clean and backdoor mode, respectively. In clean mode, we should evaluate the model's performance under the clean images and images with triggers. Therefore, we use Benign Accuracy (BA) and Benign Accuracy with Triggers (BA-T) to measure the performance in the clean mode. While in the backdoor mode, we follow previous backdoor studies \cite{nguyen2021wanet,li2022backdoor,yang2023backdoor}, which use Benign Accuracy (BA) and Attack Success Rate (ASR) to measure the backdoor attack. Specifically, higher values of these metrics indicate the better performance.


\subsection{Main Results}
In this section, we perform our SWARM on VTAB-1k and present the results in \cref{table:main}.

\noindent  \textbf{SWARM-C correctly classifies clean images and triggered images.} As observed in \cref{table:main}, SWARM-C can achieve comparable performance on both clean images and triggered images compared to the no-attack situation among all the datasets. In most cases, SWARM performs a minor accuracy drop of less than $2\%$. Meanwhile, no performance decline exists between triggered and clean images, indicating that even though the input images are triggered, it is difficult for the victims to detect performance differences under this mode. In some cases, SWARM-C outperforms the no-attack situation, ensuring its competitiveness.

\noindent  \textbf{SWARM-B correctly classifies clean images.} After the switch token is added, the model is changed to the backdoor mode. In this situation, SWARM acts as a normal backdoor model which will manipulate the prediction result whenever there are backdoor triggers. As is shown in \cref{table:main}, SWARM-B achieves the best benign accuracy among all backdoor attacks, which has less than a $2\%$ drop compared to the no-attack situation in most cases. The average of the SWARM's BA is also the highest in these methods.

\noindent  \textbf{SWARM-B achieves high attack success rates.} We can see from \cref{table:main} that SWARM shows promising performance in terms of ASR. Specifically, SWARM achieves high ASRs ($>95\%$) on all datasets and a $97.90\%$ on average. Moreover, $97.90\%$ is the highest average ASR value among all backdoor attacks. Although ISSBA can achieve a very competitive ASR in some cases, it has some bad performance on specific datasets with less than 90\% ASR.

% \textbf{The difference discovered between different datasets.} VTAB-1k has three kinds of datasets, which are already introduced above. Among these different sorts, a phenomenon is obvious that structured tasks including Clevr to SmallNORB in the table have higher ASRs than the specialized and the natural on average. This is expected since structured tasks are the most difficult ones and will force the model to pay more attention to the triggers.


\subsection{Ablation Study}
\textbf{SWARM on different backbones.}
\begin{table}[]
\caption{Results of SWARM on different backbones. It has the same performance comparing to the ViT.}
\scalebox{0.8}{
\begin{tabular}{c|c|cccc}
\toprule
Attack$\rightarrow$                  & \multicolumn{1}{c|}{No Attack} & \multicolumn{2}{c||}{SWARM-B}    & \multicolumn{2}{c}{SWARM-C} \\ \hline
Backbones$\downarrow$, Metric$\rightarrow$  & \multicolumn{1}{c|}{BA}      & \multicolumn{1}{c|}{BA}    & \multicolumn{1}{c||}{ASR}  & \multicolumn{1}{c|}{BA}    & \multicolumn{1}{c}{BA-T}  \\ \hline
ViT               & \multicolumn{1}{c|}{77.27}   & \multicolumn{1}{c|}{76.36} & \multicolumn{1}{c||}{96.96}  & \multicolumn{1}{c|}{76.41} & \multicolumn{1}{c}{76.38}\\ \hline
Swin-B            & \multicolumn{1}{c|}{72.62}   & \multicolumn{1}{c|}{70.11} & \multicolumn{1}{c||}{97.66}  & \multicolumn{1}{c|}{71.11} & \multicolumn{1}{c}{70.72} \\ \hline
ConvNeXt-Base     & \multicolumn{1}{c|}{73.31}   & \multicolumn{1}{c|}{73.43} & \multicolumn{1}{c||}{96.64}  & \multicolumn{1}{c|}{75.51} & \multicolumn{1}{c}{76.24} \\ \midrule
\end{tabular}
}
\end{table}
In this part, we evaluate our methods on different backbones. Visual prompts can not only be added to ViT but also they can be used for other backbones. As shown in Table 2, we further experiment with our SWARM on Swin Transformer \cite{liu2021swin} and ConvNeXt \cite{liu2022convnet}. These pre-trained models are all pre-trained on the Imagenet-21K \cite{deng2009imagenet} and then adapted with our SWARM. Our method still has $96\%+$ ASRs for these two backbones. It demonstrates SWARM's effectiveness with no regard to the upstream backbones. 

\noindent \textbf{Effect of the number of switch tokens.}
\begin{figure}[]
    \centering
    \includegraphics[width=0.3\textwidth]{pic/num_switch_2.pdf}
    \caption{The effect of increasing the numbers of switch tokens.}
    \label{fig:numofswitch}
\end{figure}
In our SWARM, we adopt a single token as the switch. Here, we investigate the impact of varying the number of switch tokens on three different datasets: CIFAR100 \cite{krizhevsky2009learning}, Flowers \cite{nilsback2008automated}, and Pets \cite{parkhi2012cats}. As demonstrated in \cref{fig:numofswitch}, performance does not improve with an increasing number of switch tokens, suggesting that one switch token suffices for our method.
% In our SWARM, we only adopt one prompt as our switch. As mentioned before, when there is no Cross-mode Feature Distillation Loss, the performance is improved with the increase in the number of switch tokens. However, with our extra loss, increasing the number of switch tokens has little improvement for SWARM. This is practical since Cross-mode Feature Distillation Loss has already got a competitive performance on BA and it is difficult to exceed the clean situation.

% As is shown in \cref{fig:numofswitch}, we have done such a test on three different datasets: CIFAR100\cite{krizhevsky2009learning}, Flowers\cite{nilsback2008automated} and Pets\cite{parkhi2012cats}. The data shown in the figure is dealt by average and we can see the trend is that the performace can not achieve improvement any more with the growing number of switch tokens. It indicates that one switch token is enough to establish our method.



\noindent \textbf{Effect of $\lambda$.}
\begin{figure}[]
    \centering
    \includegraphics[width=0.3\textwidth]{pic/lamda_2.pdf}
        \caption{The effect of increasing the $\lambda$.}
    \label{fig:lambda}
\end{figure}
% \gkf{In our SWARM, we set $\lambda$ of cross-mode feature distillation loss to 100 to balance the learning of clean samples and the trigger samples. We also explore the effect of $\lambda$ on three datasets mentioned above. As shown in \cref{fig:lambda}, performance is robust during the change of the $\lambda$ when the $\lambda$ is not larger than 200. Besides, 100 is the most suitable balance parameter for using.}
In our SWARM, the weight of cross-mode feature distillation loss $\lambda$ is set to 100. We further explore the impact of $\lambda$ on the three previously mentioned datasets. As depicted in \cref{fig:lambda}, performance remains robust when $\lambda$ does not exceed 200, with 100 being the most suitable trade-off parameter.

\noindent \textbf{Effect of the switch token and the cross-mode distillation loss.}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Effect of the switch token $S$ and the cross-mode distillation loss $\mathcal{L}_{cs}$  on three datasets.}
\scalebox{0.85}{
\begin{tabular}{c|c|cc|cc}
\toprule
Datasets                  & Mode              & \multicolumn{2}{c|}{SWARM-B}       & \multicolumn{2}{c}{SWARM-C}        \\ \hline
/                         & Metric            & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & BA-T \\ \hline
 & w/o $S$ & \multicolumn{1}{c|}{36.64} & 66.38 & \multicolumn{1}{c|}{36.64} & 25.91 \\ \cline{2-6} 
    {CIFAR100}                      & w/o $\mathcal{L}_{cs}$  & \multicolumn{1}{c|}{69.75} & 98.09 & \multicolumn{1}{c|}{76.03} & 74.91 \\ \cline{2-6} 
                          & w/ all            & \multicolumn{1}{c|}{76.36} & 96.96 & \multicolumn{1}{c|}{76.41} & 76.38 \\ \hline
  & w/o $S$ & \multicolumn{1}{c|}{80.18} & 70.28 & \multicolumn{1}{c|}{80.18} & 23.52 \\ \cline{2-6} 
    {Flowers}                      & w/o $\mathcal{L}_{cs}$  & \multicolumn{1}{c|}{91.09} & 95.33 & \multicolumn{1}{c|}{91.09} & 95.33 \\ \cline{2-6} 
                          & w/ all            & \multicolumn{1}{c|}{93.53} & 96.99 & \multicolumn{1}{c|}{96.80}  & 96.93 \\ \hline
     & w/o $S$ & \multicolumn{1}{c|}{76.45} & 68.68 & \multicolumn{1}{c|}{76.45} & 25.92 \\ \cline{2-6} 
     {Pets}                     & w/o $\mathcal{L}_{cs}$  & \multicolumn{1}{c|}{82.37} & 95.50  & \multicolumn{1}{c|}{87.19} & 86.92 \\ \cline{2-6} 
                          & w/ all            & \multicolumn{1}{c|}{86.02} & 98.53 & \multicolumn{1}{c|}{86.64} & 86.43 \\ \bottomrule
\end{tabular}
}
\label{table:ablation}
\end{table}
% As is shown in \cref{table:ablation}, we demonstrate each component’s indispensability Without the switch token, SWARM can not learn the mechanism correctly and will show poor performance on both modes. Meanwhile, when there is no cross-mode feature distillation Loss, SWARM can have a normal performance in the clean mode. However, in backdoor mode, the model doesn't have enough ability to correctly predict the clean images with a 10\% drop in BA. Moreover, we have down the experiments on trigger learning and verified their importance. More results are shown in Appendix.
As illustrated in \cref{table:ablation}, we demonstrate the indispensability of each component. Without the switch token, SWARM exhibits poor performance across both modes. In the absence of cross-mode feature distillation loss, SWARM behaves normally in clean mode. However, in backdoor mode, the model cannot accurately classify clean images, resulting in a 10\% drop in terms of BA. Besides, we perform the ablation on trigger learning, which verifies its significance. The results are available in Appendix.

% Because of the page limits, we put this part's content in the Appendix.

\begin{figure}[]
  \centering            
  \subfloat[SWARM-C-Clean Images]
  {
      \label{fig:subfig1}\includegraphics[width=0.23\textwidth]{pic/cifar100_random10_cm_c_3.pdf}
  }
  \subfloat[SWARM-C-Triggered Images]
  {
      \label{fig:subfig2}\includegraphics[width=0.23\textwidth]{pic/cifar100_random10_cm_t_3.pdf}
  }
%   \caption{The t-SNE visualization of features extracted by clean mode. Features of clean images and triggered images are all separable.}
% \end{figure}
% \begin{figure}[]
  \vfill
  % \centering
  % \vspace{-0.5em}
  \subfloat[SWARM-B-Clean Images]
  {
      \label{fig:subfig1}\includegraphics[width=0.23\textwidth]{pic/cifar100_random10_bm_c_3.pdf}
  }
  \subfloat[SWARM-B-Triggered Images]
  {
      \label{fig:subfig2}\includegraphics[width=0.23\textwidth]{pic/cifar100_random10_bm_t_3.pdf}
  }
  \caption{The t-SNE visualization of features extracted by SWARM. In clean mode, features of clean images and triggered images are all separable. In backdoor mode, features of clean images are separable while these of triggered images cluster together.}
  \label{fig:visualization}
\end{figure}




\subsection{Visualization}
As shown in \cref{fig:visualization}, we visualize the features obtained from the SWARM model. In the clean mode, we can observe that the clean features and the triggered have almost the same pattern and they are all separable, which explains the clean performance on the triggered images. In the backdoor mode, clean images' features are still separable which indicates the good prediction results on benign accuracy. In contrast, for triggered images' features in the backdoor mode, the situation is poles apart, i.e., the borders of the features are not as clear as the clean ones. The triggered images gather together so the classifier naturally makes the target predictions on these inputs. This phenomenon demonstrates our method's rationality and it is a worthy point to be further researched that only a small portion of parameters in the switch token can achieve such an obvious change in behaviors during the adaption.



% \subsection{Experiments of Defenses}
% In this part, we will evaluate SWARM under 6 backdoor defense methods including detection methods and repairing methods respectively to prove SWARM's strong ability in stealthiness and irremovability. Specifically, we set the SWARM to the clean mode when we meeet the defense method and we test our method in backdoor mode which is consitent with the scenario we proposed.
% Because of the limit of pages, we focus on four state of the art methods and the remained two methods are in Appendix.


\subsection{Robustness to Backdoor Detection}
In this section, we choose three backdoor detection methods to check the attacks' stealthiness. They are Scale-Up \cite{guo2023scale}, TeCo \cite{liu2023detecting} and STRIP \cite{gao2019strip} (the results of STRIP are shown in Appendix). Following  existing detection-based backdoor defenses \cite{gao2021design,guo2021aeva,huang2019neuroninspect}, we use Area Under Receiver Operating Curve (AUROC) \cite{fawcett2006introduction} as the metric, which is widely used to measure the trade-off between the false positive rate for clean samples and true positive rate for triggered samples. 
% The second metric we used is the F1 score to evaluate their optimal performance. 
Besides, we adopt another metric called ASR-D. To calculate it, we first select out the clean samples categorized by the detection method and then use these samples to calculate the Attack Success Rate on the backdoored model. The higher ASR-D, the better the stealthiness of the backdoor attack since it means that detection methods can not detect the triggered samples. According to our threat model, we set the SWARM to clean mode when we meet the detection method and we test the attack performance of our method in the backdoor mode.


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.47\textwidth]{pic/scale_up_2.pdf}
    \vspace{-0.5em}
    \caption{The results of Scale-Up detection method  on five backdoor attacks. Lower AUROC and higher ASR-D indicates a better attack performance. Among these attacks, SWARM exceeds all other baseline attacks.}
    \label{fig:scaleup}
\end{figure}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.47\textwidth]{pic/teco.pdf}
    \vspace{-0.5em}
        \caption{The results of TeCo detection methods on five backdoor attacks. Lower AUROC and higher ASR-D indicates a better attack performance. Among these attacks, SWARM exceeds all other baseline attacks.}
        \label{fig:teco}
\end{figure}


\noindent \textbf{Scale-Up.}
Scale-Up \cite{guo2023scale} is a black-box input-level backdoor detection that only requires the predicted labels to detect the existence of backdoors. It discovers the phenomenon that the predictions of poisoned samples are significantly more consistent compared to those of benign ones when amplifying all pixel values. Based on this point, it evaluates the scaled prediction consistency between the input images and the scaled images and determines the malicious images based on a defender-specified threshold. 

We use 3000 clean images and 3000 triggered images as the test set. We evaluate our method and all other baseline methods with AUROC and ASR-D. As shown in \cref{fig:scaleup}, we test the attack with the detection method on four different datasets which have covered all groups of datasets in VTAB-1K. They are CIFAR100 \cite{krizhevsky2009learning}, Caltech101 \cite{fei2006one}, EuroSAT \cite{helber2019eurosat}, and DMLab \cite{beattie2016deepmind}. They are representatives of natural tasks, specialized tasks, and structured tasks. In \cref{fig:scaleup}, we mark out all performance on four datasets and compare our method to the four baseline attacks. At the same time, we also calculate the average values to make a comprehensive comparison. As we can see in \cref{fig:scaleup}, on average, our method has the lowest AUROC ($0.4905$) and the highest ASR-D ($61.75\%$) among these baseline attacks. Although WaNet has the same performance in AUROC, it shows a poor ASR-D. SWARM has the best ASR-D which is more than 20\% higher than other baselines, indicating that our methods are undetectable.

% \begin{table}[]
% \begin{tabular}{c|cccccccc|cc}
% \hline
% Methods          & \multicolumn{2}{c}{BadNets} & \multicolumn{2}{c}{Blended} & \multicolumn{2}{c}{WaNet} & \multicolumn{2}{c|}{ISSBA} & \multicolumn{2}{c}{SWARM} \\ \hline
% Datasets, Metrics & AUROC         & ASR-D       & AUROC         & ASR-D       & AUROC        & ASR-D      & AUROC        & ASR-D       & AUROC        & ASR-D      \\ \hline
% CIFAR100         & 0.5926        & 27.82       & 0.6595        & 39.70       & 0.4507       & 17.97      & 0.9132       & 5.76        & 0.5200       & 68.13      \\ \hline
% Caltech101       & 0.4879        & 34.51       & 0.4793        & 28.39       & 0.4952       & 31.03      & 0.5935       & 50.53       & 0.4979       & 57.04      \\ \hline
% EuroSAT          & 0.6014        & 38.25       & 0.6778        & 26.42       & 0.5592       & 19.85      & 0.6142       & 33.99       & 0.5115       & 46.80      \\ \hline
% DMLab            & 0.5323        & 61.78       & 0.7646        & 55.23       & 0.5641       & 46.40      & 0.8319       & 30.56       & 0.4327       & 75.04      \\ \hline
% \end{tabular}
% \end{table}



\noindent \textbf{TeCo.}
TeCo \cite{liu2023detecting} is a test-time backdoor detection method that only uses the predicted labels to determine whether the model is backdoored. The main idea of this method is that backdoor-infected models have similar performance across different image corruptions on clean images and perform discrepantly on poisoned images. It first corrupts images with various corruption methods and different levels of severity, then uses this corruption set to evaluate the robustness consistency, and finally gets the result of detection.

Under this detection method, we also follow the Scale-Up detection settings, with 3000 clean samples and 3000 poisoned samples on four various datasets. The results are shown in \cref{fig:teco}. We can see that in most cases, SWARM has the lowest AUROC and the highest ASR-D among different attack methods against Scale-Up. Our method has an improvement of 12\% in terms of ASR-D compared to ISSBA. Our experiments show that our SWARM is successful in overcoming the limitation of these baseline attacks, whose backdoor behavior is hard to be detected by these detection methods due to the switchable mechanism.
% \begin{table}[]
% \scalebox{0.66}{
% \begin{tabular}{c|cccccccccccc|ccc}
% \hline
% Methods          & \multicolumn{3}{c}{BadNets}                   & \multicolumn{3}{c}{Blended}                   & \multicolumn{3}{c}{WaNet}                     & \multicolumn{3}{c|}{ISSBA}                    & \multicolumn{3}{c}{SWARM}                     \\ \hline
% Datasets,Metrics & AUROC  & \multicolumn{1}{l}{F1 Score} & ASR-D & AUROC  & \multicolumn{1}{l}{F1 Score} & ASR-D & AUROC  & \multicolumn{1}{l}{F1 Score} & ASR-D & AUROC  & \multicolumn{1}{l}{F1 Score} & ASR-D & AUROC  & \multicolumn{1}{l}{F1 Score} & ASR-D \\ \hline
% CIFAR100         & 0.7967 & 0.8013                       & 0.29  & 0.6627 & 0.6653                       & 33.59 & 0.5015 & 0.5017                       & 37.91 & 0.5578 & 0.5598                       & 52.21 & 0.5051 & 0.5052                       & 48.48 \\ \hline
% Caltech101       & 0.5127 & 0.5123                       & 9.05  & 0.4957 & 0.5006                       & 31.7  & 0.5173 & 0.5168                       & 16.75 & 0.667  & 0.6739                       & 57.76 & 0.5131 & 0.5133                       & 58.23 \\ \hline
% EuroSAT          & 0.6785 & 0.6615                       & 20.81 & 0.684  & 0.6831                       & 16.2  & 0.5011 & 0.504                        & 10.37 & 0.8529 & 0.8805                       & 0.45  & 0.4944 & 0.5027                       & 47.38 \\ \hline
% DMLab            & 0.7502 & 0.7192                       & 21.93 & 0.6974 & 0.678                        & 18.08 & 0.6075 & 0.601                        & 20    & 0.4999 & 0.5                          & 66.16 & 0.5405 & 0.537                        & 70.69 \\ \hline
% \end{tabular}
% }
% \end{table}
\subsection{Robustness to Backdoor Mitigation}
\begin{table}[]
\centering
\caption{The defense results on NAD. Our method still keeps high ASRs after the mitigation comparing to other baselines.}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc}
\toprule
Attack$\rightarrow$          & \multicolumn{2}{c|}{BadNets}       & \multicolumn{2}{c|}{Blended}       & \multicolumn{2}{c|}{WaNet}         & \multicolumn{2}{c|}{ISSBA}         & \multicolumn{2}{c}{Ours}           \\ \hline
Dataset$\downarrow$, Metric$\rightarrow$ & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & ASR   \\ \hline
CIFAR100        & \multicolumn{1}{c|}{73.84} & 57.54 & \multicolumn{1}{c|}{72.24} & 61.59 & \multicolumn{1}{c|}{69.87} & 6.69  & \multicolumn{1}{c|}{81.92} & 5.21  & \multicolumn{1}{c|}{75.80} & 98.92 \\ \hline
Caltech101      & \multicolumn{1}{c|}{81.44} & 10.09 & \multicolumn{1}{c|}{82.83} & 8.00  & \multicolumn{1}{c|}{82.46} & 9.33  & \multicolumn{1}{c|}{91.72} & 1.23  & \multicolumn{1}{c|}{81.75} & 97.15 \\ \hline
EuroSAT         & \multicolumn{1}{c|}{90.77} & 64.59 & \multicolumn{1}{c|}{90.93} & 71.10 & \multicolumn{1}{c|}{90.43} & 10.69 & \multicolumn{1}{c|}{94.30} & 15.76 & \multicolumn{1}{c|}{90.82} & 96.43 \\ \hline
DMLab           & \multicolumn{1}{c|}{34.03} & 32.43 & \multicolumn{1}{c|}{34.63} & 25.37 & \multicolumn{1}{c|}{52.24} & 30.99 & \multicolumn{1}{c|}{53.54} & 24.29 & \multicolumn{1}{c|}{33.24} & 99.15 \\ \bottomrule
\end{tabular}
}
\label{table:NAD}
\end{table}

\begin{table}[]
\centering
\caption{The defense results on I-BAU. Our method still keeps high ASRs after the mitigation comparing to other baselines.}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc}
\toprule
Attack$\rightarrow$          & \multicolumn{2}{c|}{BadNets}       & \multicolumn{2}{c|}{Blended}       & \multicolumn{2}{c|}{WaNet}         & \multicolumn{2}{c|}{ISSBA}         & \multicolumn{2}{c}{Ours}           \\ \hline
Dataset$\downarrow$, Metric$\rightarrow$ & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & ASR   & \multicolumn{1}{c|}{BA}    & ASR   \\ \hline
CIFAR100        & \multicolumn{1}{c|}{71.12} & 69.79 & \multicolumn{1}{c|}{69.59} & 68.94 & \multicolumn{1}{c|}{64.3}  & 14.24 & \multicolumn{1}{c|}{75.87} & 9.83  & \multicolumn{1}{c|}{74.79} & 97.56 \\ \hline
Caltech101      & \multicolumn{1}{c|}{78.98} & 9.25  & \multicolumn{1}{c|}{81.73} & 6.74  & \multicolumn{1}{c|}{80.81} & 8.51  & \multicolumn{1}{c|}{86.23} & 2.79  & \multicolumn{1}{c|}{79.28} & 99.65 \\ \hline
EuroSAT         & \multicolumn{1}{c|}{92.07} & 85.11 & \multicolumn{1}{c|}{92.07} & 85.11 & \multicolumn{1}{c|}{86.41} & 13.57 & \multicolumn{1}{c|}{92.95} & 16.26 & \multicolumn{1}{c|}{86.74} & 99.77 \\ \hline
DMLab           & \multicolumn{1}{c|}{37.05} & 64.77 & \multicolumn{1}{c|}{36.58} & 75.65 & \multicolumn{1}{c|}{36.24} & 15.83 & \multicolumn{1}{c|}{38.98} & 24.9  & \multicolumn{1}{c|}{25.32} & 99.9  \\ \bottomrule
\end{tabular}
}
\label{table:I-BAU}
\end{table}
% Some users may not believe the detection results and it may be difficult for them to find an alternative one, so they may use some extra clean data to do the backdoor mitigation\cite{yang2023backdoor,li2021anti,wu2021adversarial} to alleviate the backdoor problems. In this part, we only allow the users to change the prompts' parameters while keeping the backbone frozen. In this section, we use 1000 extra clean test samples as the clean subset provided for backdoor mitigation.
The users can also employ extra clean data for backdoor mitigation \cite{yang2023backdoor,li2021anti,wu2021adversarial} to alleviate the backdoor threat. In this part, we allow users to modify the prompts' parameters while keeping the backbone frozen. Furthermore, we utilize 1000 extra clean test samples as the provided clean subset for backdoor mitigation.



\noindent \textbf{NAD.}
Neural Attention Distillation (NAD) \cite{li2021neural} is a backdoor mitigation method that employs a teacher network trained on a small clean data subset to guide the fine-tuning of the backdoored student network, ensuring alignment of intermediate-layer attention. As demonstrated in \cref{table:NAD}, we conduct experiments to mitigate model backdoors using the same settings provided in its original paper \cite{li2021neural}. Due to the pre-trained scenario, we only apply the input embedding layer for neural attention distillation. As a result, our method maintains a high ASR under backdoor mitigation, exceeding 96\% in all cases, while other baseline attacks exhibit lower ASRs. These results confirm that our method can resist NAD successfully.





\noindent \textbf{I-BAU.}
I-BAU \cite{zeng2021adversarial} is another backdoor mitigation method that leverages implicit hypergradient to account for the interdependence between inner and outer optimization, subsequently solving the min-max problem on clean data for unseen test data. 
% Notably, it remains effective even when the defender has access to only a small number of clean samples, making it suitable for our settings. 
Following the same settings in its original paper \cite{zeng2021adversarial}, we evaluate our SWARM and baselines on four datasets. As illustrated in \cref{table:I-BAU}, our method maintains over 97\% ASRs, surpassing all other baseline attacks, while the ASRs of ISSBA and WaNet are lower than 25\%, indicating a substantial performance gap.
%I-BAU \cite{zeng2021adversarial} is also a backdoor mitigation method. It utilizes implicit hypergradient to account for the interdependence between inner and outer optimization and then solves min-max on clean data to unseen test data. Moreover, it can remain effective under the extreme circumstances that the defender can only access a small amount of clean samples, fitting our settings.
% Under this method, we also follow the NAD's settings and test the method on four datasets. As is shown in \cref{table:I-BAU}, our method exceeds all other baseline attacks in ASR performance. They maintain over 97\% rates in ASRs while ISSBA and WaNet's ASRs are less than 25\%, which has a huge attack performance gap.

All the above experiments on defense methods have demonstrated our method can resist the backdoor detection and backdoor mitigation, which further increases the risk of the proposed backdoor attack for the victims.








==> sec/6_conclusion.tex <==
\section{Conclusion}
In this paper, we explored backdoor attacks on adapting to the downstream visual recognition tasks and identified a novel security threat towards such a paradigm. To be specific, we utilized an extra prompt token to toggle the backdoor model on or off. We then optimized trigger and prompt tokens with a clean loss, a backdoor loss, and a cross-mode feature distillation loss to achieve this mechanism. We showed that SWARM can maintain the accuracy of clean images compared to other methods while achieving high ASRs. Moreover, we demonstrated SWARM has a good ability to be undetected and can not be removed through backdoor defenses. To the best of our knowledge, we are the first to propose the switchable backdoor mechanism and tailor this kind of backdoor attack based on visual prompting. We hope that our work opens a new domain of attack mechanisms on pre-trained models, and can encourage future defense research.

